South Pointing Chariot: An Invitation to Differential Geometry

We introduce the south-pointing chariot, an intriguing mechanical device from ancient China. We use its ability to keep track of a global direction as it travels on an arbitrary path as a tool to explore the geometry of curved surfaces. This takes us as far as a famous result of Gauss on the impossibility of a faithful map of the globe, which started off the field of differential geometry. The reader should get a view into how geometers think and an introduction to important early results in the field, but should need no more than a solid background in calculus (ideally through multivariable calculus). This is achieved by relying on the reader's visual intuition.

==> macros.tex <==
\usepackage{latexsym,amsmath, amssymb,ulem}
%
%
%
\newcounter{draft} % 1 means draft, 0 means publishable
\setcounter{draft}{1} % 1 means draft, 0 means publishable
%
%
%%\input{/Volumes/WORK/Helper/gaugetheory.sty}
\ifnum \thedraft=0
\addtolength{\textwidth}{1in}
\addtolength{\oddsidemargin}{-.5in}
\addtolength{\evensidemargin}{-.5in}
\fi
\makeatletter
\def\subsection{\@startsection {subsection}{2}{\z@}{.8ex
plus 1ex} {1ex}{\sc}}
\makeatother
\newenvironment{proof}{\vspace*{2ex}\noindent {\em Proof:}
}{\hfill $\Box$ \\[2ex]}
%\newenvironment{proof}{}{}
\newcommand{\new}{\newcommand}
%\renewcommand{\baselinestretch}{2}
\newcounter{letter}
\newenvironment{alist}{
\begin{list}{{\upshape(\alph{letter})}}{\usecounter{letter}}
}{\end{list}}
%\new{\sout}[1]{}
\new{\Nabla}{\bigtriangledown}
\new{\Ricci}{\mathrm{Ricci}}
\new{\Pfaff}{\mathrm{Pfaff}}
\new{\Hom}{\mathrm{Hom}}
\new{\MQ}{\mathrm{K}^{\mathrm{qm}}}
\new{\Path}{\mathrm{Path}}
\new{\kernel}{\mathrm{Kernel}}
\new{\boxtensor}{\boxtimes}
\new{\barpsi}{\overline{\psi}}
\new{\barrho}{\overline{\rho}}
\new{\iso}{\cong}
\new{\vol}{\operatorname{Vol}}
\new{\End}{\mathrm{End}}
%\new{\id}{\mathbf{1}}
\new{\grad}{\mathrm{grad}}
\new{\diverge}{\mathrm{div}}
\new{\tr}{\mathrm{tr}}
\new{\indx}{\mathrm{ind}}
\new{\str}{\mathrm{str}}
\new{\Str}{\mathrm{Str}}
%\new{\op}{\mathrm{op}}
\new{\scalar}{{\mathfrak{r}}}
\new{\kk}{{\mathfrak{k}}}
\new{\lop}{{\mathfrak{l}}}
\new{\defequals}{\stackrel{\mathrm{def}}{=}}
\new{\NN}{\mathbb{N}}
\new{\RR}{\mathbb{R}}
\new{\ZZ}{\mathbb{Z}}
\renewcommand{\v}{v}
\newcommand{\w}{w}
\renewcommand{\vector}{\mathbf}
\renewcommand{\vec}{\vector}
\new{\ltilde}{\tilde{L}}
\new{\gap}{{\;}}
\new{\depends}[1]{{\scriptscriptstyle{#1\!\!}}}
\new{\triplegap}{{\;\;\;\;\;}}
\new{\doublegap}{{\;\;\;}}
%\new{\LL}{{\mathcal{L}}}
\new{\FF}{{\mathcal{F}}}
\new{\Alg}{{\mathcal{A}}}
\new{\bundle}{{\mathcal{E}}}
\new{\QQ}{{\mathcal{Q}}}
\new{\CC}{{\mathcal{C}}}
\new{\OO}{{\mathcal{O}}}
\new{\EE}{{\mathcal{E}}}
\new{\D}{{\mathcal{D}}}
\new{\Lie}{{\mathcal{L}}}
\new{\dd}{{\mathfrak{d}}}
\new{\tensor}{\otimes}
\new{\bracket}[1]{\left\langle #1 \right \rangle}
\new{\parens}[1]{\!\left( #1 \right)}
\new{\sbrace}[1]{\!\left[ #1 \right]}
\new{\cbrace}[1]{\!\left\{ #1 \right\}}
\new{\abs}[1]{\left| #1 \r|}
%\new{\superterm}[1]{{\left\lfloor #1 \right\rfloor}}
\new{\pt}{\mathfrak{P}}
%\new{\pt}{\overline{P}}
\new{\bint}{\oint}
%\new{\hol}{\mathrm{Hol}}
%\new{\spin}{\mbox{Spin}}
\new{\pfend}{\noindent \hfill $\Box$}
\new{\beas}{\begin{eqnarray*}}
\new{\eeas}{\end{eqnarray*}}
\renewcommand{\r}{\right}
\renewcommand{\l}{\left}
\new{\norm}[1]{\l|\!\l| #1 \r|\!\r|}
%give it title and label.  Prints label with title in draft mode
\new{\para}[2]{\subsection{#1. }
\label{par:#2} \ifnum \thedraft=1 \marginpar{\scriptsize{par:#2}} \fi}
%
%give it label.  prints label in draft mode.
\new{\be}{\begin{equation}  
}
\new{\ee}[1]{%ref
\label{eq:#1}
\end{equation} \ifnum \thedraft=1 \marginpar{\scriptsize{\em{eq:#1}}}  
\fi \noindent%
}
%give it label.  prints label in draft mode.
\new{\eqa}[2]{\begin{align}
#2 \label{eq:#1}
\end{align}
\ifnum \thedraft=1 \marginpar{\scriptsize{\em{eq:#1}}}  \fi
}
%label within eqnarrays that prints in draft mode -- had to give this
%up because we're inside an environment that is not considered
%"(outer) paragraph mode"
\new{\eqalabel}[1]{
\label{eq:#1}
%\ifnum \thedraft=1 \marginpar{\scriptsize{\em{eq:#1}}} \fi
}
%label that behaves right in draft mode
\new{\dlabel}[1]{\ifnum \thedraft=1 \marginpar{\scriptsize{\em{#1}}}  \fi}
%
%label for equations as items
\new{\labitem}[1]{%
\label{item:#1} \ifnum \thedraft=1 \marginpar{\scriptsize{\em{item:#1}}}  
\fi \noindent%
}
\numberwithin{equation}{section}
\newtheorem{remark}{Remark}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{definition}{Definition}
